Adversarial Attacks on Stochastic Bandits

We study adversarial attacks that manipulate the reward signals to control the actions chosen by a stochastic multi-armed bandit algorithm. We propose the first attack against two popular bandit algorithms: $\epsilon$-greedy and UCB, \emph{without} knowledge of the mean rewards. The attacker is able to spend only logarithmic effort, multiplied by a problem-specific parameter that becomes smaller as the bandit problem gets easier to attack. The result means the attacker can easily hijack the behavior of the bandit algorithm to promote or obstruct certain actions, say, a particular medical treatment. As bandits are seeing increasingly wide use in practice, our study exposes a significant security threat.

==> an-linucb.tex <==
\section{Offline Attack on Contextual Bandit}

We now turn our attention to the offline attack of contextual bandit. In particular, we consider attacking LinUCB\cite{li10contextual,abbasi11improved}, a linear contextual bandit that is widely used due to its practical efficiency. Assume there are $K$ arms, and each arm is associated with a parameter $\theta_i\in \mathbb{R}^d(1\le i\le K)$. The reward of pulling arm $i$ is $x^\top \theta_i+\eta$, where $x$ $(\lVert x\rVert \le S)$ is the context and $\eta$ is a $\sigma^2$-sub-Gaussian random noise. Let $X_i\in \mathbb{R}^{N_i(t-1)\times d}$ be the matrix whose rows are the contexts where arm $i$ is pulled up to round $t$-1, and use $r_i\in \mathbb{R}^{N_i(t-1)}$ to denote the corresponding rewards. In round $t$, the arm that LinUCB selects to pull is $I_t=\arg\max_{i\in K} (x_t^\top\hat\theta_i+\gamma_i\lVert  x_t\rVert_{\bar V_i^{-1}})$, where $\bar V_i=X_i^\top X_i+\lambda I$, $\hat \theta_i=(X_i^\top X_i+\lambda I)^{-1} X_i^\top r_i$ is an estimate for $\theta_i$ using ridge regression with penalization $\lambda$, $x_t$ is the context at round $t$, $\gamma_i=\sigma^2\sqrt{2\log (\frac{\text{det}(\bar V_i)^\frac{1}{2}\text{det}(\lambda I)^{-\frac{1}{2}}}{\delta})}$, and $\lVert  x_t\rVert_{\bar V_i^{-1}}=\sqrt{x_t^\top \bar V_i^{-1}x_t}$.

To illustrate the attack protocol, consider the recommendation system of news articles. The system has a pool of articles (arms) that can be displayed online. Each time a user (represented by a context) comes, the system selects an article based on its recommendation policy. The selected article is then displayed to the user and the system receives reward, corresponding to whether the article was clicked by the user or not. Whenever the system runs for a period of time, its policy will be updated. The attacker has in mind a group of target users, e.g. all those belonging to the republic party, and a target article which may look extremely attractive to the republicans. The attacker then sneaks inside the system right before the rule is updated, manipulating all previous rewards so that after the attack, if any republican comes, the system will display the target article.

Let $X^*$ be the target group of contexts and $i^*$ be the target article. Different from the online attack which is performed continuously, the offline attack only happens at particular rounds since the bandit updates its policy periodically. Let $t$ be a round when attack happens. The attacker manipulates all previous rewards up to round $t-1$, namely $r_i$ $(1\le i\le K)$, such that after the attack, if any target context $x\in X^*$ appears, the bandit will always pull the target arm $i^*$.

Let $\alpha_i\in \mathbb{R}^{N_{i}(t-1)}$ be the attack vector for arm $i$, then the rewards of arm $i$ after attack is $r_i-\alpha_i$. To ensure that $i^*$ is selected for any $x\in X^*$, the following condition must be satisfied:
\begin{equation}
\begin{aligned}
&x^\top\bar V_{i^*}^{-1} X_{i^*}^\top (r_{i^*}-\alpha_{i^*})+\gamma_{i^*}\lVert x\rVert_{\bar V_{i^*}^{-1}}\\
&\ge  \epsilon+x^\top\bar V_i^{-1} X_i^\top (r_i-\alpha_i)+\gamma_i\lVert x\rVert_{\bar V_i^{-1}},\\
& \forall i\neq i^*\text{ and } \forall x\in X^*.\\
\end{aligned}
\end{equation}

where $\epsilon>0$ guarantees separation. Meanwhile, we hope that the attack vector has small magnitude in order to avoid detection, thus the overall attack can be modeled as the following optimization problem:
\begin{equation}\label{attack:OFUL_multi}
\begin{aligned}
\min_{} & \sum_{i\in [K]} \lVert \alpha_i \rVert_2\\
\text{s.t. } &x^\top\bar V_{i^*}^{-1} X_{i^*}^\top (r_{i^*}-\alpha_{i^*})+\gamma_{i^*}\lVert x\rVert_{\bar V_{i^*}^{-1}}\\
&\ge  \epsilon+x^\top\bar V_i^{-1} X_i^\top (r_i-\alpha_i)+\gamma_i\lVert x\rVert_{\bar V_i^{-1}},\\
& \forall i\neq i^*\text{ and } \forall x\in X^*.\\
\end{aligned}
\end{equation}
The $\ell_2$-norm in the objective is not critical - one can replace it with any norm of interest to derive solution with desirable properties such as sparseness. The following lemma shows that~\eqref{attack:OFUL_multi} is also convex.
\begin{lem}
The optimization problem~\eqref{attack:OFUL_multi} is convex.
\end{lem}
\begin{proof}
Let $\alpha=(\alpha_1;\alpha_2;...\alpha_K)\in \mathbb{R}^{t-1}$, which is a vector constructed by stacking $\alpha_i$ in one column. Let $f_x(\alpha)=x^\top\bar V_{i^*}^{-1} X_{i^*}^\top (r_{i^*}-\alpha_{i^*})+\gamma_{i^*}\lVert x\rVert_{\bar V_{i^*}^{-1}}
 - \epsilon-x^\top\bar V_i^{-1} X_i^\top (r_i-\alpha_i)+\gamma_i\lVert x\rVert_{\bar V_i^{-1}}$. The feasible region of~\eqref{attack:OFUL_multi} is $\cap_{x\in X^*}\{\alpha: f_x(\alpha)\ge 0\}$. Note that $f_x(\alpha)$ is concave (also convex) in $\alpha$, thus $\{\alpha: f_x(\alpha)\ge 0\}$ is convex for all $x$. Also note that the intersection of convex sets remains convex, thus $\cap_{x\in X^*}\{\alpha: f_x(\alpha)\ge 0\}$ is convex, i.e. the feasible region is convex. It is clear that the objective is also a convex function of $\alpha$, thus the overall problem is convex.
 
\subsection{Simulation on Synthetic Data}

(show synthetic experiment result)

\subsection{Experiment on Yahoo! User Click Log Dataset}

We attack the LinUCB on Yahoo! user click log dataset~\citep[R6A]{YahooWebscopeToday}, which contains a fraction of user click log to the Featured Tab of the Today Module in Yahoo! Front Page\cite{} during the first ten days in May 2009. The total number of user visits is 45,811,883 and are divided into 5-minute windows. In each window, the number of the articles that can be displayed is around 20 and remains stable for 5 minutes.
\end{proof}

